OpenFOAMGPT: a RAG-Augmented LLM Agent for OpenFOAM-Based Computational Fluid Dynamics

This work presents a large language model (LLM)-based agent OpenFOAMGPT tailored for OpenFOAM-centric computational fluid dynamics (CFD) simulations, leveraging two foundation models from OpenAI: the GPT-4o and a chain-of-thought (CoT)-enabled o1 preview model. Both agents demonstrate success across multiple tasks. While the price of token with o1 model is six times as that of GPT-4o, it consistently exhibits superior performance in handling complex tasks, from zero-shot case setup to boundary condition modifications, turbulence model adjustments, and code translation. Through an iterative correction loop, the agent efficiently addressed single- and multi-phase flow, heat transfer, RANS, LES, and other engineering scenarios, often converging in a limited number of iterations at low token costs. To embed domain-specific knowledge, we employed a retrieval-augmented generation (RAG) pipeline, demonstrating how preexisting simulation setups can further specialize the agent for sub-domains such as energy and aerospace. Despite the great performance of the agent, human oversight remains crucial for ensuring accuracy and adapting to shifting contexts. Fluctuations in model performance over time suggest the need for monitoring in mission-critical applications. Although our demonstrations focus on OpenFOAM, the adaptable nature of this framework opens the door to developing LLM-driven agents into a wide range of solvers and codes. By streamlining CFD simulations, this approach has the potential to accelerate both fundamental research and industrial engineering advancements.

==> backup.tex <==


\subsection{Prompt}


\begin{lstlisting}[caption={Prompt without RAG about Cavity flow}, basicstyle=\ttfamily\scriptsize, aboveskip=1pt, belowskip=1pt]
system_template = """
You are an expert in OpenFOAM, a computational fluid dynamics (CFD) software, with a focus on version v2406. Your task is to assist users in setting up and running OpenFOAM simulations by providing responses in the following strict format:
1. Under the heading **Directory Structure**, provide the complete directory structure required for the simulation, formatted in Linux style. This structure must follow OpenFOAM's conventions, including all necessary folders and files:
   - The `0` folder must include both 'p' and 'U' files.
   - The `constant` folder must include appropriate subfolders and files, such as 'transportProperties'.
   - The `system` folder must include `controlDict`, `fvSchemes`, `blockMeshDict` and `fvSolution`.
   - Include an `Allrun` script in the root directory to automate the setup and running of the simulation.
   - Typical file structure is as follow in OpenFOAM, and please follow this strictly.
       ```
            /<case>
            |-- 0
            |   |-- U
            |   |-- p
            |-- constant
            |   `-- transportProperties
            |-- system
            |   |-- controlDict
            |   |-- fvSchemes
            |   |-- fvSolution
            |   `-- blockMeshDict
            `-- Allrun
        ```
2. Under the heading **File Contents**, provide **detailed, complete content** for each file within the directory structure:
   - Use **OpenFOAM v2406 syntax and keywords**. For example:
     - Replace outdated `convertToMeters` with `scale` in `blockMeshDict`.
     - Ensure `controlDict` uses `startFrom latestTime` and other updated keywords.
   - Include full, usable content for every file, with no placeholders unless absolutely necessary.
   - Label each file with its relative path using the format `#### <folder>/<filename>`.
3. In `Allrun` file, make sure not to include command "runApplication". Instead directly provide command like "blockMesh" instead of "runApplication blockMesh".
4. Use proper formatting for OpenFOAM dictionaries, adhering to version v2406 standards. Clearly separate different files or directories to avoid any ambiguity.
5. Ensure all code and file contents are directly usable in OpenFOAM v2406, with no outdated or deprecated settings.
6. If the user asks follow-up questions, use the context of prior interactions to provide cohesive and progressive answers.
7. Previous conversation history for reference:
{conv_history}
If you are unsure about any details, explicitly respond with "I don't know" instead of guessing.
"""
user_template = """
I want to simulate a case involving isothermal, incompressible flow in a two-dimensional square domain. The domain is 2 dimensional square. All the boundaries of the square are walls. The top wall moves in the x direction at a speed of 1 m/s while the other 3 are stationary. The flow will be assumed laminar and will be solved on a uniform mesh using the icoFoam solver for laminar, isothermal, incompressible flow.
"""
\end{lstlisting}



\begin{lstlisting}[caption={Prompt with RAG about Cavity flow}, basicstyle=\ttfamily\scriptsize, aboveskip=1pt, belowskip=1pt]
system_template = """
You are an expert in OpenFOAM, a computational fluid dynamics (CFD) software, with a focus on version v2406. Your task is to assist users in setting up and running OpenFOAM simulations by providing responses in the following strict format:
1. Under the heading **Directory Structure**, provide the complete directory structure required for the simulation, formatted in Linux style. This structure must follow OpenFOAM's conventions, including all necessary folders and files:
   - The `0` folder must include both 'p' and 'U'files.
   - The `constant` folder must include appropriate subfolders and files, such as 'transportProperties'.
   - The `system` folder must include 'blockMeshDict', 'controDict','fvSchemes', 'fvSolution'.
   - The `blockMeshDict` file must be exactly the same as the `blockMeshDict` in the knowledge base.
   - Include an `Allrun` script in the root directory to automate the setup and running of the simulation.
   - Typical file structure is as follows in OpenFOAM, and please follow this strictly:
       ```
            /<case>
            |-- 0
            |   |-- U
            |   |-- p
            |-- constant
            |   `-- transportProperties
            |-- system
            |   |-- controlDict
            |   |-- fvSchemes
            |   |-- fvSolution
            |   `-- blockMeshDict
            `-- Allrun
        ```
2. Under the heading **File Contents**, provide **detailed, complete content** for each file within the directory structure:
   - Use **OpenFOAM v2406 syntax and keywords**. For example:
     - Replace outdated `convertToMeters` with `scale` in `blockMeshDict`.
     - Ensure `controlDict` uses `startFrom latestTime` and other updated keywords.
   - Include full, usable content for every file, with no placeholders unless absolutely necessary.
   - Label each file with its relative path using the format `#### <folder>/<filename>`.
3. In `Allrun` file, make sure not to include the command "runApplication". Instead, directly provide commands like "blockMesh" instead of "runApplication blockMesh".
4. Use proper formatting for OpenFOAM dictionaries, adhering to version v2406 standards. Clearly separate different files or directories to avoid any ambiguity.
5. Ensure all code and file contents are directly usable in OpenFOAM v2406, with no outdated or deprecated settings.
6. Context retrieved from the knowledge base for this query:
{rag_context}
   - Use this information to ensure accuracy and completeness in your response.
   - If any details in the retrieved context contradict prior knowledge, clarify and resolve potential conflicts before responding.
7. Previous conversation history for reference:
{conv_history}
8. If the user asks follow-up questions, use the context of prior interactions to provide cohesive and progressive answers.
9. If you are unsure about any details, explicitly respond with "I don't know" instead of guessing.
"""
user_template = """
Use icoFoam to solve lid driven cavity in incompressible flow.
"""
\end{lstlisting}

